TimeStep Master: Asymmetrical Mixture of Timestep LoRA Experts for Versatile and Efficient Diffusion Models in Vision

Diffusion models have driven the advancement of vision generation over the past years. However, it is often difficult to apply these large models in downstream tasks, due to massive fine-tuning cost. Recently, Low-Rank Adaptation (LoRA) has been applied for efficient tuning of diffusion models. Unfortunately, the capabilities of LoRA-tuned diffusion models are limited, since the same LoRA is used for different timesteps of the diffusion process. To tackle this problem, we introduce a general and concise TimeStep Master (TSM) paradigm with two key fine-tuning stages. In the fostering stage (1-stage), we apply different LoRAs to fine-tune the diffusion model at different timestep intervals. This results in different TimeStep LoRA experts that can effectively capture different noise levels. In the assembling stage (2-stage), we design a novel asymmetrical mixture of TimeStep LoRA experts, via core-context collaboration of experts at multi-scale intervals. For each timestep, we leverage TimeStep LoRA expert within the smallest interval as the core expert without gating, and use experts within the bigger intervals as the context experts with time-dependent gating. Consequently, our TSM can effectively model the noise level via the expert in the finest interval, and adaptively integrate contexts from the experts of other scales, boosting the versatility of diffusion models. To show the effectiveness of our TSM paradigm, we conduct extensive experiments on three typical and popular LoRA-related tasks of diffusion models, including domain adaptation, post-pretraining, and model distillation. Our TSM achieves the state-of-the-art results on all these tasks, throughout various model structures (UNet, DiT and MM-DiT) and visual data modalities (Image, Video), showing its remarkable generalization capacity.

==> tabs/distill_abla.tex <==
\begin{table}[t]
\centering
\begin{minipage}[t]{0.9\linewidth}
    \vspace{0pt}
    \centering
    \belowrulesep=0pt\aboverulesep=0pt
    \captionsetup{font=normalsize}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|l|l}
        \toprule
        \textbf{Metric} & \textbf{FT Method} 
         & \textbf{Value} 
         \\
        
        \midrule
        % \multirow{9}{*}{\shortstack[c]{DMD2}} 

        \multirow{3}{*}{\shortstack[c]{FID$\downarrow$}} 
        & Vanilla LoRA
        & 14.58
        \\
        & TSM 1-stage & 9.92 \quad
 \textcolor{darkGreen}{$\downarrow$ 4.66} \\
        & TSM 2-stage & 9.90 \quad \textcolor{darkGreen}{$\downarrow$ 4.68} 
        \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{Patch \\-FID$\downarrow$}} 
        & Vanilla LoRA
        & 15.43
        \\
        & TSM 1-stage & 11.88 \ \ \textcolor{darkGreen}{$\downarrow$ 3.55} \\
        & TSM 2-stage & 11.82 \ \ 
        \textcolor{darkGreen}{$\downarrow$ 3.61} 
        \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{CLIP- \\ Score$\uparrow$}} 
        & Vanilla LoRA
        & 0.3176 
        \\
        & TSM 1-stage & 0.3208 \textcolor{darkGreen}{$\uparrow$ \%1.01} \\
        & TSM 2-stage & 0.3212 \textcolor{darkGreen}{$\uparrow$ \%1.13}
        % 0.3042，
        \\
        
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.3cm}
    \caption{\textbf{Model Distillation Ablation based on DMD2.}}
    
    \vspace{-0.3cm}
    \label{tab:distill_abla_new}
\end{minipage}
\vspace{-0.42cm}
\end{table}

==> tabs/domain_ada_abla+distill_abla+domain_ada_router+post_pre_abla.tex <==
\begin{table*}[t]
\centering
% 使用 minipage 并排放置两个表格
\begin{minipage}[t]{0.71\textwidth}
    \centering
    \Large  % 如果需要大字体，可以加在这里
    \setlength\tabcolsep{4pt}
    \renewcommand{\arraystretch}{0.8}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{clllllll}
        \toprule
        \textbf{Model}
         & \textbf{FT Method}
         & \textbf{Color$\uparrow$} 
         & \textbf{Shape$\uparrow$} 
         & \textbf{Texture$\uparrow$} 
         & \textbf{Spatial$\uparrow$} 
         & \textbf{Non-Spatial$\uparrow$}
         & \textbf{Complex$\uparrow$}\\
        \midrule
        \multirow{3}{*}{\shortstack[c]{SD1.5 \\ UNet}} 
        & Vanilla LoRA & 51.57 & 44.76 & 52.68 & 15.45 & 31.69 & 32.83 \\
        & TSM 1-stage & 56.48\textcolor{darkGreen}{$\uparrow$ 4.91} 
                      & 45.91\textcolor{darkGreen}{$\uparrow$ 1.15} 
                      & 57.08\textcolor{darkGreen}{$\uparrow$ 5.12}
                      & 18.01\textcolor{darkGreen}{$\uparrow$ 2.56}
                      & 31.77\textcolor{darkGreen}{$\uparrow$ 0.08}
                      & 32.79\textcolor{red}{$\downarrow$ 0.04} \\
        & TSM 2-stage & 57.12\textcolor{darkGreen}{$\uparrow$ 5.55} 
                      & 46.65\textcolor{darkGreen}{$\uparrow$ 1.89} 
                      & 58.16\textcolor{darkGreen}{$\uparrow$ 5.48} 
                      & 18.80\textcolor{darkGreen}{$\uparrow$ 3.35}
                      & 31.83\textcolor{darkGreen}{$\uparrow$ 0.14}
                      & 32.94\textcolor{darkGreen}{$\uparrow$ 0.11} \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{PixArt-$\alpha$ \\ DiT}} 
        & Vanilla LoRA & 46.53 & 43.75 & 53.37 & 23.08 & 30.97 & 34.75 \\
        & TSM 1-stage & 52.84\textcolor{darkGreen}{$\uparrow$ 6.31} 
                      & 43.92\textcolor{darkGreen}{$\uparrow$ 0.17}
                      & 54.07\textcolor{darkGreen}{$\uparrow$ 0.70} 
                      & 25.35\textcolor{darkGreen}{$\uparrow$ 2.27}
                      & 31.03\textcolor{darkGreen}{$\uparrow$ 0.06}
                      & 35.04\textcolor{darkGreen}{$\uparrow$ 0.29} \\
        & TSM 2-stage & 54.66\textcolor{darkGreen}{$\uparrow$ 8.13} 
                      & 44.47\textcolor{darkGreen}{$\uparrow$ 0.72}
                      & 57.12\textcolor{darkGreen}{$\uparrow$ 3.75}
                      & 25.41\textcolor{darkGreen}{$\uparrow$ 2.33}
                      & 31.05\textcolor{darkGreen}{$\uparrow$ 0.08}
                      & 34.85\textcolor{darkGreen}{$\uparrow$ 0.10} \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{SD3 \\ MM-DiT}} 
        & Vanilla LoRA & 82.41 & 62.32 & 77.27 & 31.87 & 31.72 & 38.41 \\
        & TSM 1-stage & 82.52\textcolor{darkGreen}{$\uparrow$ 0.11}
                      & 62.94\textcolor{darkGreen}{$\uparrow$ 0.62}
                      & 77.55\textcolor{darkGreen}{$\uparrow$ 0.28}
                      & 33.08\textcolor{darkGreen}{$\uparrow$ 1.21}
                      & 31.74\textcolor{darkGreen}{$\uparrow$ 0.02}
                      & 38.54\textcolor{darkGreen}{$\uparrow$ 0.13} \\
        & TSM 2-stage & 83.45\textcolor{darkGreen}{$\uparrow$ 1.04}
                      & 63.16\textcolor{darkGreen}{$\uparrow$ 0.84}
                      & 78.18\textcolor{darkGreen}{$\uparrow$ 0.91}
                      & 34.50\textcolor{darkGreen}{$\uparrow$ 2.63}
                      & 31.81\textcolor{darkGreen}{$\uparrow$ 0.09}
                      & 38.71\textcolor{darkGreen}{$\uparrow$ 0.30} \\
        \bottomrule
    \end{tabular}
    } 
    \vspace{-0.4cm}
    \caption{\textbf{Domain Adaptation Ablation on T2I-CompBench.}}
    \label{table: domain_ada_abla}
\end{minipage}%
\hfill
\begin{minipage}[t]{0.284\textwidth}
    \centering
    \Large  % 如果需要大字体，也可放在这里
    \belowrulesep=0pt\aboverulesep=0pt
    \captionsetup{font=normalsize}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|l|l}
        \toprule
        \textbf{Metric} & \textbf{FT Method} & \textbf{Value} \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{FID$\downarrow$}} 
         & Vanilla LoRA & 14.58 \\
         & TSM 1-stage  & 9.92 \quad \textcolor{darkGreen}{$\downarrow$ 4.66} \\
         & TSM 2-stage  & 9.90 \quad \textcolor{darkGreen}{$\downarrow$ 4.68} \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{Patch \\-FID$\downarrow$}}
         & Vanilla LoRA & 15.43 \\
         & TSM 1-stage  & 11.88 \quad \textcolor{darkGreen}{$\downarrow$ 3.55} \\
         & TSM 2-stage  & 11.82 \quad \textcolor{darkGreen}{$\downarrow$ 3.61} \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{CLIP- \\ Score$\uparrow$}} 
         & Vanilla LoRA & 0.3176 \\
         & TSM 1-stage  & 0.3208 \textcolor{darkGreen}{$\uparrow$ \%1.01} \\
         & TSM 2-stage  & 0.3212 \textcolor{darkGreen}{$\uparrow$ \%1.13} \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-0.4cm}
    \caption{\textbf{Model Distillation Ablation based on DMD2.}}
    \label{tab:distill_abla_new}
\end{minipage}

\vspace{-0.15cm}
\hspace{-0.2cm}
\begin{minipage}[t]{0.37\linewidth}
    \vspace{0pt}  % 让它顶端对齐
    \renewcommand{\arraystretch}{0.7}
    \centering
    \Large
    % \setlength\tabcolsep{4pt} % 可根据需要启用
    % 尽量不要在这里再加 \vspace{-0.3cm} 这样的负间距
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{cccccccccc}
            \toprule
            \textbf{Model}
             & $z_{t}$ & $t$
             & \textbf{Col$\uparrow$} 
             & \textbf{Sha$\uparrow$} 
             & \textbf{Tex$\uparrow$} 
             & \textbf{Spa$\uparrow$} 
             & \textbf{NS$\uparrow$}
             & \textbf{Com$\uparrow$}\\
            \midrule
            \multirow{3}{*}{\shortstack[c]{SD1.5 \\ UNet}} 
            & \cmark & \cmark & \textbf{57.12} & \textbf{46.65} & \textbf{58.16} & \textbf{18.80} & \textbf{31.83} & 32.94 \\
            & \xmark & \cmark & 51.42 & 44.09 & 53.46 & 13.56 & 31.75 & \textbf{33.45} \\
            & \cmark & \xmark & 53.64 & 46.24 & 55.08 & 16.31 & 31.72 & 33.42 \\
            \midrule
            \multirow{3}{*}{\shortstack[c]{PixArt-$\alpha$ \\ DiT}} 
            & \cmark & \cmark & \textbf{54.66} & 44.47 & \textbf{57.12} & \textbf{25.41} & \textbf{31.05} & 34.85 \\
            & \xmark & \cmark & 45.37 & 42.49 & 52.09 & 24.84 & 30.99 & 34.83 \\
            & \cmark & \xmark & 47.23 & \textbf{44.69} & 54.30 & 25.25 & 30.99 & \textbf{34.86} \\
            \midrule
            \multirow{3}{*}{\shortstack[c]{SD3 \\ MM-DiT}} 
            & \cmark & \cmark & \textbf{83.45} & \textbf{63.16} & \textbf{78.18} & \textbf{34.50} & \textbf{31.81} & 38.71 \\
            & \xmark & \cmark & 80.99 & 60.38 & 74.62 & 31.87 & 31.61 & 38.53 \\
            & \cmark & \xmark & 82.55 & 62.25 & 76.68 & 31.53 & 31.74 & \textbf{38.87} \\
            \bottomrule
        \end{tabular}
    }
    \vspace{-0.4cm}
    \caption{\textbf{Gating Ablation on T2I-CompBench.}
    Performance is optimal when inputs both $z_{t}$ and $t$.}
    \label{table: domain_ada_router}
\end{minipage}%
% \hfill
%============== 右侧表格 ==============
\hspace{0.2cm}
\begin{minipage}[t]{0.62\linewidth}
    \vspace{0.265cm}
    \renewcommand{\arraystretch}{1}
    \centering
    \Large
    \setlength\tabcolsep{4pt}
    % 同样尽量避免这里的负间距
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{clllllll}
            \toprule
            \textbf{IMG Model} & \textbf{FT Method} 
             & \textbf{Color$\uparrow$} 
             & \textbf{Shape$\uparrow$} 
             & \textbf{Texture$\uparrow$} 
             & \textbf{Spatial$\uparrow$} 
             & \textbf{Non-Spatial$\uparrow$}
             & \textbf{Complex$\uparrow$}\\
            \midrule
            \multirow{3}{*}{\shortstack[c]{PixArt-$\alpha$}} 
            & Vanilla LoRA & 43.47 & 34.74 & 41.57 & 15.37 & 30.74 & 30.43 \\
            & TSM 1-stage & 45.66 \textcolor{darkGreen}{$\uparrow$ 2.19} & 37.06 \textcolor{darkGreen}{$\uparrow$ 2.32} & 45.42 \textcolor{darkGreen}{$\uparrow$ 3.85} & 22.32 \textcolor{darkGreen}{$\uparrow$ 6.95} & 31.03 \textcolor{darkGreen}{$\uparrow$ 0.29} & 32.65 \textcolor{darkGreen}{$\uparrow$ 2.22} \\
            & TSM 2-stage & 48.86 \textcolor{darkGreen}{$\uparrow$ 5.39} & 37.97 \textcolor{darkGreen}{$\uparrow$ 3.23} & 47.31 \textcolor{darkGreen}{$\uparrow$ 5.74} & 16.18 \textcolor{darkGreen}{$\uparrow$ 1.66} & 31.13 \textcolor{darkGreen}{$\uparrow$ 0.39} & 32.96 \textcolor{darkGreen}{$\uparrow$ 2.53} \\
            \toprule
            \textbf{VID Model} &
             \textbf{FT Method}
             & \textbf{IS$\uparrow$}
             & \textbf{Action$\uparrow$}
             & \textbf{Amplitude$\uparrow$}
             & \textbf{BLIP-BLEU$\uparrow$} 
             & \textbf{Color$\uparrow$}
             & \textbf{Count$\uparrow$} \\
            \midrule
            \multirow{3}{*}{\shortstack[c]{VC2}} 
            & Vanilla LoRA & 15.06 & 73.85 & 46.0 & 21.89 & 41.30 & 27.89 \\
            & TSM 1-stage & 16.71 \textcolor{darkGreen}{$\uparrow$ 1.65}  & 79.07 \textcolor{darkGreen}{$\uparrow$ 5.22} & 50.0 \textcolor{darkGreen}{$\uparrow$ 4.0} & 23.99 \textcolor{darkGreen}{$\uparrow$ 2.10} & 56.52 \textcolor{darkGreen}{$\uparrow$ 15.22} & 55.48 \textcolor{darkGreen}{$\uparrow$ 27.59} \\
            & TSM 2-stage & 18.08 \textcolor{darkGreen}{$\uparrow$ 3.02} & 80.77 \textcolor{darkGreen}{$\uparrow$ 6.92} & 54.0 \textcolor{darkGreen}{$\uparrow$ 8.0} & 24.26 \textcolor{darkGreen}{$\uparrow$ 2.37} & 60.87 \textcolor{darkGreen}{$\uparrow$ 19.57} & 60.38 \textcolor{darkGreen}{$\uparrow$ 32.49} \\
            \bottomrule
        \end{tabular}
    }
    \vspace{-0.4cm}
    \caption{\textbf{Image and Video Post-Pretraining Ablation on T2I-CompBench and EvalCrafter.}}
    \label{table: post_pre_abla}
\end{minipage}

\end{table*}

==> tabs/domain_ada_para.tex <==
\begin{table}[!ht]
\belowrulesep=0pt\aboverulesep=0pt
    \renewcommand{\arraystretch}{1}
    \centering
    \setlength\tabcolsep{1pt}
    \resizebox{0.47\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c}
        \toprule
        \rule{0pt}{0.3cm}
        \textbf{Model}
         & \textbf{Method} 
         & \textbf{Diffusion Network} 
         & \textbf{Text Encoder} 
         & \textbf{Trainable (\%)}  \\
        \midrule

        SD1.5 & Vanilla LoRA & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (0.7972M) & $W_{q}$, $W_{v}$ (0.1475M) & 0.09604\\
        \hhline{~|-|-|-|-}
        UNet & TM 1-stage & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (0.7972M) & $W_{q}$, $W_{v}$ (0.1475M) & 0.09604\\
        \hhline{~|-|-|-|-}
        ~ & TM 2-stage & $R_{q}$, $R_{k}$, $R_{v}$, $R_{out}$ (0.2275M) & $R_{q}$, $R_{v}$ (0.04243M) & 0.02722 \\
        \hhline{-|-|-|-|-}

        PixArt-$\alpha$ & Vanilla LoRA & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (0.2064M) & $W_{q}$, $W_{v}$ (0.1573M) & 0.06764\\
        \hhline{~|-|-|-|-}
        DiT & TM 1-stage & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (0.2064M) & $W_{q}$, $W_{v}$ (0.1573M) & 0.06764\\
        \hhline{~|-|-|-|-}
        ~ & TM 2-stage & $R_{q}$, $R_{k}$, $R_{v}$, $R_{out}$ (0.0482M) & $R_{q}$, $R_{v}$ (0.02446M) & 0.01344 \\
        \hhline{-|-|-|-|-}

        SD3 & Vanilla LoRA & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (1.18M) & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (1.606M) & 0.05635\\
        \hhline{~|-|-|-|-}
        MM-DiT & TM 1-stage & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (1.18M) & $W_{q}$, $W_{k}$, $W_{v}$, $W_{out}$ (1.606M) & 0.05635\\
        \hhline{~|-|-|-|-}
        ~ & TM 2-stage & $R_{q}$, $R_{k}$, $R_{v}$, $R_{out}$ (0.2435M) & $R_{q}$, $R_{k}$, $R_{v}$, $R_{out}$ (0.3767M) & 0.01311 \\
        \bottomrule

        
    \end{tabular}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Comparison of Trainable Parameters.} 
    $W$ and $R$ represent the trainable LoRA and Router in TSM. 
    The trainable parameters in 1-stage is equal to vanilla LoRA. 
    In 2-stage, 
    the trainable parameters are approximately 1/4 of those in 1-stage. }
    \label{table: domain_ada_para}
\vspace{-0.14cm}
\end{table}

==> tabs/domain_ada_router.tex <==
\begin{table}[t]
\centering
\begin{minipage}[t]{0.9\linewidth}
    \vspace{0pt}
    \renewcommand{\arraystretch}{0.7}
    \centering
    \captionsetup{font=normalsize}
    % \setlength\tabcolsep{4pt}
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{cccccccccc}
        \toprule
        \textbf{Model}
         & $z_{t}$ & $t$
         & \textbf{Color$\uparrow$} 
         & \textbf{Shape$\uparrow$} 
         & \textbf{Texture$\uparrow$} 
         & \textbf{Spatial$\uparrow$} 
         & \textbf{Non-Spatial$\uparrow$}
         & \textbf{Complex$\uparrow$}\\
        \midrule
        \multirow{3}{*}{\shortstack[c]{SD1.5 \\ UNet}} 
        & \cmark & \cmark & \textbf{57.12} & \textbf{46.65} & \textbf{58.16} & \textbf{18.80} & \textbf{31.83} & 32.94 \\
        & \xmark & \cmark & 51.42 & 44.09 & 53.46 & 13.56 & 31.75 & \textbf{33.45} \\
        & \cmark & \xmark & 53.64 & 46.24 & 55.08 & 16.31 & 31.72 & 33.42 \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{PixArt-$\alpha$ \\ DiT}} 
        & \cmark & \cmark & \textbf{54.66} & 44.47 & \textbf{57.12} & \textbf{25.41} & \textbf{31.05} & 34.85 \\
        & \xmark & \cmark & 45.37 & 42.49 & 52.09 & 24.84 & 30.99 & 34.83 \\
        & \cmark & \xmark & 47.23 & \textbf{44.69} & 54.30 & 25.25 & 30.99 & \textbf{34.86} \\
        \midrule
        \multirow{3}{*}{\shortstack[c]{SD3 \\ MM-DiT}} 
        & \cmark & \cmark & \textbf{83.45} & \textbf{63.16} & \textbf{78.18} & \textbf{34.50} & \textbf{31.81} & 38.71 \\
        & \xmark & \cmark & 80.99 & 60.38 & 74.62 & 31.87 & 31.61 & 38.53 \\
        & \cmark & \xmark & 82.55 & 62.25 & 76.68 & 31.53 & 31.74 & \textbf{38.87} \\
        \bottomrule
    \end{tabular}
    }
    % \caption{\textbf{Domain Adaptation Ablation on T2I-CompBench.} 
    % }
    \vspace{-0.3cm}
    \caption{\textbf{Gating Ablation on T2I-CompBench.}
    The model performance is optimal when the router's input has both $z_{t}$ and $t$.
    }
    \label{table: domain_ada_router}
\end{minipage}
\vspace{-0.42cm}
\end{table}
